TrackFormer: Multi-Object Tracking with Transformers

The challenging task of multi-object tracking (MOT) requires simultaneous reasoning about track initialization, identity, and spatio-temporal trajectories. We formulate this task as a frame-to-frame set prediction problem and introduce TrackFormer, an end-to-end trainable MOT approach based on an encoder-decoder Transformer architecture. Our model achieves data association between frames via attention by evolving a set of track predictions through a video sequence. The Transformer decoder initializes new tracks from static object queries and autoregressively follows existing tracks in space and time with the conceptually new and identity preserving track queries. Both query types benefit from self- and encoder-decoder attention on global frame-level features, thereby omitting any additional graph optimization or modeling of motion and/or appearance. TrackFormer introduces a new tracking-by-attention paradigm and while simple in its design is able to achieve state-of-the-art performance on the task of multi-object tracking (MOT17 and MOT20) and segmentation (MOTS20). The code is available at https://github.com/timmeinhardt/trackformer .

==> figures/simulate_MOT.tex <==
\begin{figure} %[ht]
    \centering
    \includegraphics[width=0.49\columnwidth]{figures/teaser}
    % \hspace{5px}
    \includegraphics[width=0.49\columnwidth]{figures/teaser}
    \label{fig:simulate_MOT}
    \caption{We simulate multi-object tracking scenarios by augmenting single images from the CrowdHuman~\cite{crowdhuman} dataset.}
\end{figure}

==> tables/ablation_ch.tex <==
\begin{table}
    \tablestyle{1.2pt}{1.05}
    \begin{center}
        \begin{tabular}[t]{lcc cc}
            \toprule
            Method           & CrowdHuman &   MOT17       & MOTA $\uparrow$ & IDF1 $\uparrow$ \\

            \midrule

            \multirow{2}{*}{CenterTrack~\cite{center_track}}        &  $\times$  &  $\times$        & 60.5 & 55.7 \\
                                                     &            &  $\times$        & 65.4 & 60.8 \\

            \multirow{2}{*}{TrackFormer}        &  $\times$  &  $\times$        & 61.5 & 59.3 \\
                                                     &            &  $\times$   &     65.0 & 63.9 \\

            \bottomrule
        \end{tabular}
    \end{center}
    %
    \caption{
        Ablation study on the performance gain from training on the CrowdHuman dataset.
        %
        We train DETR~\cite{DETR} only for object detection and associate tracks based on output embedding distance.
        %
        The first row corresponds to the last row in~\tabref{tab:ablation_study}.
        %
        \todo{public detections. no effect on detection. IoU filtering.}
    }
    %
    \label{tab:ablation_ch}
\end{table}


==> tables/ablation_detection.tex <==
\begin{table}
    % \vspace{0.35cm}
    \tablestyle{1.2pt}{1.05}
    \begin{center}
        \begin{tabular}[t]{lHH ccc}
            \toprule
            Method                  & MOT17         & CrowdHuman    & AP $\uparrow$ & FP $\downarrow$ & FN $\downarrow$\\

            \midrule

            DPM~\cite{dpmpami2009}                     &  $\times$     &  $\times$     & 0.61 & 42308 & 36557\\
            FRCNN~\cite{rennips2015}                   &  $\times$     &               & 0.72 & 10081 & 25963\\
            SDP~\cite{sdpYangcvpr2016}                     &  $\times$     &               & 0.81 & 7599 & 18865\\

            \midrule
            CenterTrack~\cite{center_track}             &  $\times$     &               & 0.77 & 7662 & 9900\\
            TrackFormer             &  $\times$     &               & 0.73 & 13178 & 15441\\

            \bottomrule
        \end{tabular}
    \end{center}
    %
    \caption{
        Detection performance on the MOT17 test set.
        %
        Both TrackFormer and CenterTrack were pretrained on CrowdHuman~\cite{crowdhuman} and evaluated only for single frame detection.
    }
    %
    \label{tab:ablation_detection}
\end{table}

==> tables/ablation_nms.tex <==
\begin{table}
    \tablestyle{1.2pt}{1.05}
    % \vspace{-10pt}
    \begin{center}
        \begin{tabular}[t]{lcc cc}
            \toprule
            Method           & NMS detection & NMS tracking                     & MOTA $\uparrow$ & IDF1 $\uparrow$ \\
            \midrule

            \multirow{3}{*}{TrackFormer}        &  $\times$  &  $\times$        & 54.6 & 53.9 \\
                                                &            &  $\times$        & 54.6 & 53.8 \\
                                                &            &                  & 51.7 & 53.0 \\

            \bottomrule
        \end{tabular}
    \end{center}
    \caption{
        Ablation study on the application of non-maximum suppression (NMS) on the set of tracks and for the detection of new objects.
        %
        The second row corresponds to the first row in~\tabref{tab:ablation_study}.
    }
    %
    \label{tab:ablation_nms}
\end{table}

==> tables/mot_eval_trackformer_seqs_center_distance.tex <==
\begin{table*}
    % \centering
    % \small

    \begin{center}
    \resizebox{0.75\textwidth}{!}{%
%    	\hspace*{-15pt}
    \begin{tabular}[t]{ll cc rrrrr H}
        \toprule
        Sequence         & Public detection                        & MOTA $\uparrow$ & IDF1 $\uparrow$ & MT $\uparrow$ & ML $\downarrow$ & FP $\downarrow$ & FN $\downarrow$ & ID Sw. $\downarrow$ & $\uparrow$ Hz \\

        \midrule

        MOT17-01 & DPM~\cite{dpmpami2009} & 51.8 & 37.7 & 8 & 6 & 436 & 2588 & 82 \\
        MOT17-03 & DPM & 75.7 & 70.0 & 104 & 12 & 8598 & 16565 & 326 \\
        MOT17-06 & DPM & 58.3 & 56.4 & 79 & 59 & 737 & 3949 & 229 \\
        MOT17-07 & DPM & 56.1 & 44.6 & 14 & 15 & 1146 & 6108 & 166 \\
        MOT17-08 & DPM & 38.9 & 35.6 & 15 & 23 & 793 & 11899 & 221 \\
        MOT17-12 & DPM & 52.3 & 58.8 & 26 & 32 & 743 & 3340 & 55 \\
        MOT17-14 & DPM & 40.5 & 42.4 & 27 & 47 & 1924 & 8595 & 484 \\

        \midrule

        MOT17-01 & FRCNN~\cite{rennips2015} & 52.0 & 39.4 & 8 & 6 & 470 & 2548 & 81 \\
        MOT17-03 & FRCNN & 76.2 & 71.1 & 103 & 12 & 8569 & 15974 & 331 \\
        MOT17-06 & FRCNN & 60.0 & 57.1 & 82 & 46 & 873 & 3590 & 248 \\
        MOT17-07 & FRCNN & 56.2 & 45.2 & 16 & 14 & 1173 & 6067 & 163 \\
        MOT17-08 & FRCNN & 36.9 & 34.9 & 14 & 25 & 811 & 12315 & 205 \\
        MOT17-12 & FRCNN & 52.4 & 58.7 & 25 & 35 & 640 & 3433 & 49 \\
        MOT17-14 & FRCNN & 38.9 & 41.0 & 28 & 44 & 2314 & 8374 & 607 \\

        \midrule

        MOT17-01 & SDP~\cite{sdpYangcvpr2016} & 55.5 & 40.4 & 9 & 4 & 478 & 2304 & 86 \\
        MOT17-03 & SDP & 75.3 & 69.8 & 105 & 12 & 10152 & 15320 & 341 \\
        MOT17-06 & SDP & 59.2 & 56.6 & 82 & 49 & 873 & 3692 & 243 \\
        MOT17-07 & SDP & 56.8 & 44.3 & 15 & 14 & 1170 & 5966 & 170 \\
        MOT17-08 & SDP & 38.1 & 35.4 & 15 & 23 & 858 & 11992 & 221 \\
        MOT17-12 & SDP & 51.9 & 60.1 & 25 & 29 & 825 & 3285 & 56 \\
        MOT17-14 & SDP & 41.1 & 41.9 & 29 & 44 & 2138 & 8158 & 594 \\

        \midrule

        All & All & 63.4 & 60.0 & 829 & 551 & 45721 & 156062 & 4958 \\

        \bottomrule
    \end{tabular}
    }
    \end{center}
    %
    \caption{
        We report the per-sequence~\textbf{TrackFormer} MOT17~\cite{MOT16} test set results with~\textbf{center distance} public detection filtering.
        %
        The results do not reflect the varying object detection performance of DPM, FRCNN and SDP, respectively.
        %
        % We apply the same ~\textbf{center distance} public detection filtering as in~\cite{center_track}.
        %
        The arrows indicate low or high optimal metric values.
    }
	\vspace{15pt}
    %
    \label{tab:mot_eval_trackformer_seqs_center_distance}
\end{table*}

==> tables/mot_splits.tex <==
\begin{table}
  \begin{center}
% \tabcolsep=0.11cm

\resizebox{\columnwidth}{!}{
  \begin{tabular}{l c c c c c}

     \toprule
     Name & CM & Length [s] & Length [f] & Tracks & Boxes \\
     \midrule
     \multicolumn{6}{c}{Split 1} \\
     \midrule
      % Name & Mov. & Length (s) & Length (f) & Tracks & Boxes \\ [0.5ex]
      MOT17-02 &        No &      20   &     600      &   62  & 18581 \\
      MOT17-10 &       Yes &      22   &     654     &   57  & 12839 \\
      MOT17-13 &       Yes &      30   &     750     &   110  & 11642 \\
      \midrule
      All &  -- &      72   &     2004     &   229  & 43062 \\
     \midrule
     \multicolumn{6}{c}{Split 2} \\
     \midrule
      % Name & Mov. & Length (s) & Length (f) & Tracks & Boxes \\ [0.5ex]
      MOT17-04 &       No   &     35    &     1050    &   83  & 47557 \\
      MOT17-11 &      Yes  &     30    &      900    &   75  & 9436 \\
      \midrule
      All &  -- &      65   &     1950     &   158  & 56993 \\
      \midrule
     \multicolumn{6}{c}{Split 3 } \\
     \midrule
      % Name & Mov. & Length (s) & Length (f) & Tracks & Boxes \\ [0.5ex]
      MOT17-05 &       Yes &      60   &     837     &   133  & 6917 \\
      MOT17-09 &       No  &      18   &     525     &   26  & 5325 \\
      \midrule
      All &  -- &      78   &     1362     &   159  & 12242 \\
     \midrule
     \multicolumn{6}{c}{Total } \\
     \midrule
      % Name & Mov. & Length (s) & Length (f) & Tracks & Boxes \\ [0.5ex]
        &       -- &      205   &   5316  &   546  &  112297 \\
     \bottomrule

    \end{tabular}
    }
  \end{center}

\caption{
  For our ablation studies, we follow the 3-fold cross-validation split on the MOT17~\cite{MOT16} training set presented in~\cite{mot_neural_solver_2020_CVPR}.
  %
  We list the respective validation sequences and indicate camera movement with~\textit{CM} and report their length in the number of seconds (s) and frames (f).
  }

\label{tab:mot_splits}

\end{table}
